Exploring the Lifecycle and Maintenance Practices of Pre-Trained Models in Open-Source Software Repositories

Pre-trained models (PTMs) are becoming a common component in open-source software (OSS) development, yet their roles, maintenance practices, and lifecycle challenges remain underexplored. This report presents a plan for an exploratory study to investigate how PTMs are utilized, maintained, and tested in OSS projects, focusing on models hosted on platforms like Hugging Face and PyTorch Hub. We plan to explore how PTMs are used in open-source software projects and their related maintenance practices by mining software repositories that use PTMs and analyzing their code-base, historical data, and reported issues. This study aims to provide actionable insights into improving the use and sustainability of PTM in open-source projects and a step towards a foundation for advancing software engineering practices in the context of model dependencies.

==> preliminary_analysis.tex <==


\begin{table*}[]
    \centering
    \begin{tabular}{p{2cm}|l l l l l}
         \textbf{Project} & \textbf{RQ1} & \textbf{RQ2} & \textbf{RQ3} & \textbf{RQ4} & \textbf{RQ5} \\ \hline
         Suno-AI/Bark  & 
        \begin{tabular}[t]{@{}l@{}}
             \textbullet\ Text-to-Voice \\ 
             \textbullet\  MIT Licence \\
             \textbullet\ Size: 300M \\
             \textbullet\ AR Transformer \\
         \end{tabular} &
         \begin{tabular}[t]{@{}l@{}}
             \textbullet\ Core Functionality \\ 
             \textbullet\ role: text-to-voice \\ 
             \textbullet\ Dynamic + Static \\ 
         \end{tabular}
         &
         \begin{tabular}[t]{@{}l@{}}
             \textbullet\ Active Maintenance \\ 
             \textbullet\ Single PTM signature \\ 
             \textbullet\ Name changed frequently \\
         \end{tabular}
         & 
         \begin{tabular}[t]{@{}l@{}}
             \textbullet\ basic testing present \\ 
             \textbullet\ No PTM-specific test \\ 
         \end{tabular}
         &
         \begin{tabular}[t]{@{}l@{}}
             \textbullet\ Many “not found” errors \\ 
             \textbullet\ +100 issues matched \\ 
         \end{tabular}\\ \hline
         
        oobabooga/text-generation-webui
        & 
        \begin{tabular}[t]{@{}l@{}} 
            \textbullet\ Supports multiple LLMs \\
            \textbullet\ AGPL-3.0 License \\
            \textbullet\ Modular architecture \\ 
            \textbullet\ Gradio-based UI \\
        \end{tabular} 
        &
        \begin{tabular}[t]{@{}l@{}} 
            \textbullet\ Core functionality \\
            \textbullet\ Role: text generation \\ 
            \textbullet\ Dynamic loading \\
        \end{tabular}
        &
        \begin{tabular}[t]{@{}l@{}} 
            \textbullet\ Active maintenance \\
            \textbullet\ Frequent updates \\
            \textbullet\ Supports various models \\ 
        \end{tabular}
        &
        \begin{tabular}[t]{@{}l@{}} 
            \textbullet\ Basic testing present \\
            \textbullet\ Limited PTM-specific tests \\
        \end{tabular}
        & 
        \begin{tabular}[t]{@{}l@{}} 
            \textbullet\ Issues with model loading \\
            \textbullet\ Compatibility errors  \\
            \textbullet\ +200 issues matched \\
        \end{tabular}\\ \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}


